Pool model: a mass preserving multi particle aggregation process

We present and study the Pool model in $\mathbb{R}^2$, a rotationally symmetric analogue of Multi-Particle Diffusion-Limited Aggregation (MDLA), in which particles ("droplets") perform continuous-time random walks and are absorbed upon entering a circular pool initially centered at the origin. Each absorbed particle increases the pool's mass, and the pool expands so that its area grows accordingly, yielding a natural mass-preserving dynamics. A central tool which is of independent interest is a version of Kurtz's theorem for this model, depicting the field of particles conditioned on the growth of the pool as an independent non-homogeneous Poisson point process.

==> imports_and_macros.tex <==
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\usepackage{amsaddr}
%\usepackage[noblocks]{authblk}
\usepackage{bm}
%\usepackage{biblatex}
\usepackage[english]{babel}
%\addbibresource{bibliography.bib}

\usepackage{latexsym,amssymb,amsmath,amsfonts,amsthm}
\usepackage{amsthm,amsmath}
\usepackage{float}
\usepackage{enumerate}
%\usepackage{epic}
\usepackage[margin=3cm]{geometry}
\usepackage{bbm}
\usepackage{subfigure}
%\usepackage{mathbbol}
\usepackage{graphicx}
\usepackage[toc,page]{appendix}
\usepackage{multirow}
\usepackage{amsfonts}
\usepackage[all]{xy}
\usepackage{caption}
\usepackage{geometry}                % See geometry.pdf to learn the layout options. There are lots.
\geometry{a4paper}                   % ... or a4paper or a5paper or ... 
%\geometry{landscape}                % Activate for for rotated page geometry
%\usepackage[parfill]{parskip}    % Activate to begin paragraphs with an empty line rather than an indent
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{epstopdf}
\usepackage{color}
\usepackage{bbm, dsfont}
%\usepackage{float}
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage[utf8]{inputenc}
\setcounter{tocdepth}{2}
%\usepackage[english]{babel}



\usepackage{amssymb,amsthm,amsmath,amssymb,wrapfig,dsfont}
\usepackage[dvipsnames]{xcolor}
\definecolor{myred}{RGB}{251,154,133}
\definecolor{myblue}{RGB}{153,206,227}
\definecolor{mylightblue}{RGB}{0, 150, 255}
\definecolor{mygreen}{RGB}{32, 210, 64}
\definecolor{mygray}{RGB}{220, 220, 220}

\usepackage{tikz}
%\usetikzlibrary{shadows}
\usetikzlibrary{decorations.pathmorphing}
\tikzset{snake it/.style={decorate, decoration=snake}}
\usetikzlibrary{shapes.geometric,positioning,decorations.pathreplacing} 

%******************packages added by Anna **********************************************
\usepackage{breqn}
\usepackage{upgreek}
\usepackage{enumitem}  

%******************packages added by Anna **********************************************

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}
\newtheorem{counterexample}{Counterexample}
\newtheorem{example}{Example}


\def\beq{ \begin{equation} }
	\def\eeq{ \end{equation} }
\def\mn{\medskip\noindent}
\def\ms{\medskip}
\def\bs{\bigskip}
\def\bn{\bigskip\noindent}
\def\ep{\varepsilon}
\def\nass{\noalign{\smallskip}}
\def\nams{\noalign{\smallskip}}
\def\square{\vcenter{\vbox{\hrule height .4pt
			\hbox{\vrule width .4pt height 5pt \kern 5pt
				\vrule width .4pt} \hrule height .4pt}}}
\def\eopt{\hfill$\square$}
\def\RR{\mathbb{R}}
\def\ZZ{\mathbb{Z}}
\def\eqd{\,{\buildrel d \over =}\,}
\def\var{\hbox{Var}\,}
\def\hbr{\hfill\break}
\def\rlh{\rightleftharpoons}

% ******************************* New commands *******************************************************
\newcommand{\BA}{{\mathbb{A}}}
\newcommand{\BB}{{\mathbb{B}}}
\newcommand{\BC}{{\mathbb{C}}}
\newcommand{\BD}{{\mathbb{D}}}
\newcommand{\BE}{{\mathbb{E}}}
\newcommand{\BF}{{\mathbb{F}}}
\newcommand{\BG}{{\mathbb{G}}}
\newcommand{\BH}{{\mathbb{H}}}
\newcommand{\BI}{{\mathbb{I}}}
\newcommand{\BJ}{{\mathbb{J}}}
\newcommand{\BK}{{\mathbb{K}}}
\newcommand{\BL}{{\mathbb{L}}}
\newcommand{\BM}{{\mathbb{M}}}
\newcommand{\BN}{{\mathbb{N}}}
\newcommand{\BO}{{\mathbb{O}}}
\newcommand{\BP}{{\mathbb{P}}}
\newcommand{\BQ}{{\mathbb{Q}}}
\newcommand{\BR}{{\mathbb{R}}}
\newcommand{\BS}{{\mathbb{S}}}
\newcommand{\BT}{{\mathbb{T}}}
\newcommand{\BU}{{\mathbb{U}}}
\newcommand{\BV}{{\mathbb{V}}}
\newcommand{\BW}{{\mathbb{W}}}
\newcommand{\BX}{{\mathbb{X}}}
\newcommand{\BY}{{\mathbb{Y}}}
\newcommand{\BZ}{{\mathbb{Z}}}


\newcommand{\FA}{{\mathfrak{A}}}
\newcommand{\FB}{{\mathfrak{B}}}
\newcommand{\FC}{{\mathfrak{C}}}
\newcommand{\FD}{{\mathfrak{D}}}
\newcommand{\FE}{{\mathfrak{E}}}
\newcommand{\FF}{{\mathfrak{F}}}
\newcommand{\FG}{{\mathfrak{G}}}
\newcommand{\FH}{{\mathfrak{H}}}
\newcommand{\FI}{{\mathfrak{I}}}
\newcommand{\FJ}{{\mathfrak{J}}}
\newcommand{\FK}{{\mathfrak{K}}}
\newcommand{\FL}{{\mathfrak{L}}}
\newcommand{\FM}{{\mathfrak{M}}}
\newcommand{\FN}{{\mathfrak{N}}}
\newcommand{\FO}{{\mathfrak{O}}}
\newcommand{\FP}{{\mathfrak{P}}}
\newcommand{\FQ}{{\mathfrak{Q}}}
\newcommand{\FR}{{\mathfrak{R}}}
\newcommand{\FS}{{\mathfrak{S}}}
\newcommand{\FT}{{\mathfrak{T}}}
\newcommand{\FU}{{\mathfrak{U}}}
\newcommand{\FV}{{\mathfrak{V}}}
\newcommand{\FW}{{\mathfrak{W}}}
\newcommand{\FX}{{\mathfrak{X}}}
\newcommand{\FY}{{\mathfrak{Y}}}
\newcommand{\FZ}{{\mathfrak{Z}}}

\newcommand{\CA}{{\mathcal{A}}}
\newcommand{\CB}{{\mathcal{B}}}
\newcommand{\CC}{{\mathcal{C}}}
\newcommand{\CD}{{\mathcal{D}}}
\newcommand{\CE}{{\mathcal{E}}}
\newcommand{\CF}{{\mathcal{F}}}
\newcommand{\CG}{{\mathcal{G}}}
\newcommand{\CH}{{\mathcal{H}}}
\newcommand{\CI}{{\mathcal{I}}}
\newcommand{\CJ}{{\mathcal{J}}}
\newcommand{\CK}{{\mathcal{K}}}
\newcommand{\CL}{{\mathcal{L}}}
\newcommand{\CM}{{\mathcal{M}}}
\newcommand{\CN}{{\mathcal{N}}}
\newcommand{\CO}{{\mathcal{O}}}
\newcommand{\CP}{{\mathcal{P}}}
\newcommand{\CQ}{{\mathcal{Q}}}
\newcommand{\CR}{{\mathcal{R}}}
\newcommand{\CS}{{\mathcal{S}}}
\newcommand{\CT}{{\mathcal{T}}}
\newcommand{\CU}{{\mathcal{U}}}
\newcommand{\CV}{{\mathcal{V}}}
\newcommand{\CW}{{\mathcal{W}}}
\newcommand{\CX}{{\mathcal{X}}}
\newcommand{\CY}{{\mathcal{Y}}}
\newcommand{\CZ}{{\mathcal{Z}}}


\newcommand{\tbA}{{\textbf{A}}}
\newcommand{\tbB}{{\textbf{B}}}
\newcommand{\tbC}{{\textbf{C}}}
\newcommand{\tbD}{{\textbf{D}}}
\newcommand{\tbE}{{\textbf{E}}}
\newcommand{\tbF}{{\textbf{F}}}
\newcommand{\tbG}{{\textbf{G}}}
\newcommand{\tbH}{{\textbf{H}}}
\newcommand{\tbI}{{\textbf{I}}}
\newcommand{\tbJ}{{\textbf{J}}}
\newcommand{\tbK}{{\textbf{K}}}
\newcommand{\tbL}{{\textbf{L}}}
\newcommand{\tbM}{{\textbf{M}}}
\newcommand{\tbN}{{\textbf{N}}}
\newcommand{\tbO}{{\textbf{O}}}
\newcommand{\tbP}{{\textbf{P}}}
\newcommand{\tbQ}{{\textbf{Q}}}
\newcommand{\tbR}{{\textbf{R}}}
\newcommand{\tbS}{{\textbf{S}}}
\newcommand{\tbT}{{\textbf{T}}}
\newcommand{\tbU}{{\textbf{U}}}
\newcommand{\tbV}{{\textbf{V}}}
\newcommand{\tbW}{{\textbf{W}}}
\newcommand{\tbX}{{\textbf{X}}}
\newcommand{\tbY}{{\textbf{Y}}}
\newcommand{\tbZ}{{\textbf{Z}}}


\newcommand{\tba}{{\textbf{a}}}
\newcommand{\tbb}{{\textbf{b}}}
\newcommand{\tbc}{{\textbf{c}}}
\newcommand{\tbd}{{\textbf{d}}}
\newcommand{\tbe}{{\textbf{e}}}
\newcommand{\tbf}{{\textbf{f}}}
\newcommand{\tbg}{{\textbf{g}}}
\newcommand{\tbh}{{\textbf{h}}}
\newcommand{\tbi}{{\textbf{i}}}
\newcommand{\tbj}{{\textbf{j}}}
\newcommand{\tbk}{{\textbf{k}}}
\newcommand{\tbl}{{\textbf{l}}}
\newcommand{\tbm}{{\textbf{m}}}
\newcommand{\tbn}{{\textbf{n}}}
\newcommand{\tbo}{{\textbf{o}}}
\newcommand{\tbp}{{\textbf{p}}}
\newcommand{\tbq}{{\textbf{q}}}
\newcommand{\tbr}{{\textbf{r}}}
\newcommand{\tbs}{{\textbf{s}}}
\newcommand{\tbt}{{\textbf{t}}}
\newcommand{\tbu}{{\textbf{u}}}
\newcommand{\tbv}{{\textbf{v}}}
\newcommand{\tbw}{{\textbf{w}}}
\newcommand{\tbx}{{\textbf{x}}}
\newcommand{\tby}{{\textbf{y}}}
\newcommand{\tbz}{{\textbf{z}}}

\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname tb\x \endcsname{\noexpand{\noexpand\textbf{\x}}}
}
\foreach \x in {a,...,z}{%
\expandafter\xdef\csname tb\x \endcsname{\noexpand{\noexpand\textbf{\x}}}
}


\newcommand{\itP}{{\textit{P}}}

\newcommand{\ind}{{\mathbbm{1}}}
\newcommand{\joint}{\Large \texttt{P}}
% ********************************** Eviatar's shortcuts ***********************************************
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
%\newcommand{\for}{{\rm for}}
\newcommand{\prob}{{\bf P}}
\newcommand{\p}{{\bf P}}
\newcommand{\e}{{\bf E}}
\newcommand{\bae}{\begin{equation}\begin{aligned}}
		\newcommand{\eae}{\end{aligned}\end{equation}}
\newcommand{\ev}{\mathbf{E}}
\newcommand{\pr}{\mathbb{P}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\cp}{\text{\bf cap}}
\newcommand{\milf}{\text{SIDLA}}
\newcommand{\dlat}{\text{DLAT}}
\newcommand{\si}{\sigma}
\newcommand{\dd}{\partial}
\newcommand{\tree}{\mathcal{T}}


\DeclareFontFamily{OML}{rsfs}{\skewchar\font'177}
\DeclareFontShape{OML}{rsfs}{m}{n}{ <5> <6> rsfs5 <7> <8> <9>
	rsfs7 <10> <10.95> <12> <14.4> <17.28> <20.74> <24.88> rsfs10 }{}
\DeclareMathAlphabet{\mathfs}{OML}{rsfs}{m}{n}


% ******************************* Greek shortcuts ******************************************************
\newcommand{\diam}{\text{diam}}
\newcommand{\high}{\textbf{high}}
\newcommand{\om}{{\omega}}
\newcommand{\dla}{\text{DLA}^\ep}
%\newcommand{\ep}{{\varepsilon}}
\newcommand{\INT}{\text{INT}}
\newcommand{\OPT}{\text{OPT}}
\newcommand{\htr}[1]{{\color{black}{{h(T(#1))}}}}

\newcommand{\note}[1]{{\color{red}{ \bf{ [Note: #1]}}}}
\DeclareMathOperator*{\esssup}{ess\,sup}
\newcommand{\rem}[1]{{\color{blue}{\bf{ #1}}}}

\newcommand{\HL}{\text{HL}}
\newcommand{\SHL}{\text{SHL}}
% ******************************* Greek shortcuts ******************************************************


\newcommand{\ima}{\text{Im}}
\newcommand{\rea}{\text{Re}}
%\newcommand{\br}{\mathfrak{B}}
\newcommand{\br}{\mathfs{B}}
%\newcommand{\htr}[1]{{\color{black}{{h(T(#1))}}}}
\newcommand{\particle}{{\Upsilon}}
%\newcommand{\diam}{\mathrm{diam}}
\newcommand{\slitN}{\slit^{N,\delta}}
\newcommand{\slitM}{\slit^{M,\delta}}
\newcommand{\slit}{\varphi}
\newcommand{\slitdelta}{\varphi^{\delta}}
\newcommand{\Ftn}{F_t^{N,\delta}}
\newcommand{\Ftnminus}{F_{t^-}^{N,\delta}}
\newcommand{\scal}{\delta (N,\lambda)}
%\newcommand{\note}[1]{{\color{red}{ \bf{ [Note: #1]}}}}
%\DeclareMathOperator*{\esssup}{ess\,sup}

% ******************************* Yam's shortcuts ******************************************************
% you can write almost all of the above commands using for loops:
% \foreach \x in {A,...,Z}{%
% \expandafter\xdef\csname cal\x \endcsname{\noexpand\ensuremath{\noexpand\mathcal{\x}}}
% }
% \foreach \x in {A,...,Z}{%
% \expandafter\xdef\csname bb\x \endcsname{\noexpand\ensuremath{\noexpand\mathcal{\x}}}
% }
\newcommand{\conncomp}[1]{CC\left(#1 \right)}  % A command for the connected component in which #1 reside
\newcommand{\T}[1]{\Tilde{#1}}
\newcommand{\EE}{\mathbb{E}}
% \newcommand{\EE}[1]{\mathbb{E}\left[ #1 \right]}

\newcommand{\Es}{\mathbf{Es}}
\newcommand{\capacity}{\operatorname{\bf cap}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\greens}[2]{\mathcal{G} \left(#1, #2 \right)}

\newcommand{\gebin}{\ge_{\text{bin}}}
\newcommand{\pibin}{\pi^{bin}}
\newcommand{\E}[1]{\mathbf{E}\left[ #1 \right]}

